The Pierre Auger Observatory Upgrade - Preliminary Design Report

The Pierre Auger Observatory has begun a major Upgrade of its already impressive capabilities, with an emphasis on improved mass composition determination using the surface detectors of the Observatory. Known as AugerPrime, the upgrade will include new 4 m$^2$ plastic scintillator detectors on top of all 1660 water-Cherenkov detectors, updated and more flexible surface detector electronics, a large array of buried muon detectors, and an extended duty cycle for operations of the fluorescence detectors. This Preliminary Design Report was produced by the Collaboration in April 2015 as an internal document and information for funding agencies. It outlines the scientific and technical case for AugerPrime. We now release it to the public via the arXiv server. We invite you to review the large number of fundamental results already achieved by the Observatory and our plans for the future.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 8371 2015-03-30 21:31:53Z engel $

USEPDFLATEX := 1
USEBIBTEX := 1

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard figs/* *.bib) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := bash
PDFS := $(addsuffix .pdf,$(TARGETS))
DEPENDENCIES += $(wildcard *.sty *.bib) Makefile

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e){print red""e""end;exit 1}}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $< ; bibtex $* ; $(LATEX) $<
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
#	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt}
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

